Are anonymity-seekers just like everybody else? An analysis of contributions to Wikipedia from Tor

User-generated content sites routinely block contributions from users of privacy-enhancing proxies like Tor because of a perception that proxies are a source of vandalism, spam, and abuse. Although these blocks might be effective, collateral damage in the form of unrealized valuable contributions from anonymity seekers is invisible. One of the largest and most important user-generated content sites, Wikipedia, has attempted to block contributions from Tor users since as early as 2005. We demonstrate that these blocks have been imperfect and that thousands of attempts to edit on Wikipedia through Tor have been successful. We draw upon several data sources and analytical techniques to measure and describe the history of Tor editing on Wikipedia over time and to compare contributions from Tor users to those from other groups of Wikipedia users. Our analysis suggests that although Tor users who slip through Wikipedia's ban contribute content that is more likely to be reverted and to revert others, their contributions are otherwise similar in quality to those from other unregistered participants and to the initial contributions of registered users.

==> ORES-to-renovate.tex <==
%%%%%RENOVATION PENDING BELOW
In the top panel of Figure \ref{}, we use non-parametric LOESS \cite{cleveland_robust_1979} curves to visualize how the average prediction that an edit is damaging changes over time.
%, and the average likelihood that an edit has been made in good faith (that is, if it's damaging, the community judges that damage to be inadvertent). 
LOESS plots are a visualization tool that use low-order polynomial regression on each datapoint to calculate a smoothed fit line which describes the data as a weighted moving average. The grey bands represent standard errors around LOESS estimates over time. 
% Because LOESS plots are non-parametric, they have the advantage of not imposing any assumptions of the distribution of the data (i.e. we do not assume a normal distribution or a linear relationship with time) and the plot can simply respond to the data we have; however this means we do not generate interpretable parameter estimates, but rather only describe the data visually. 
Because of the bursty nature of the Tor edit volume, our data is not distributed evenly over time. The bottom colored area of each subplot shows the density of data over time---solid colors indicate more data and lighter colors indicate less.
%The gray ribbon at the end of the trend lines and the thinner data evidenced at the left end of the rug on each plot is a product of the smaller sample size of edits from 2015 to 2018.  
These plots show that edits by Tor editors are similar to those by IP editors and those by first-time editors in terms of quality. The top half panel of Figure \ref{fig:ores-enwikitypes} predicts whether or not an edit made by a user in one of our groups is with good faith and tells a similar story. Tor users' behavior is similar to the IP editors and the first-time editors groups. Compared with the registered editors, it is worse.

\begin{figure*}[t]
\centering
\includegraphics[width=15cm, height=12cm]{figures/byTypeFacet.pdf}
\caption{ORES prediction of damaging and good faith edits by contributor type, drawn as a non-parametric LOESS curve.}
\label{fig:}
\end{figure*}

To provide a statistical test of the differences between the groups shown in Figure \ref{fig:ores-enwikitypes}, we fit two logistic regression models on our measures of quality with the editor group as our independent variable.  Table \ref{tab:regression-dg} reports the coefficients from this analysis with 95\% confidence intervals in brackets.  We estimated a model using fixed effect controls for month and found the results substantively unchanged.
%In the good faith model, ORES tries to assess whether the individual appears to be trying to make a contribution based on good intention (not vandal), even if their contribution is in some way erroneous, while in the damaging model, ORES tries to detect edits that may harm the article, including mistakes in formatting, well-intentioned but unwelcome additions, and deliberate damage. 

The good faith analysis shown in the first column suggests that the difference between Tor users and IP users in this model is not statistically significant. Our model predicts that 71.1\% of edits made by Tor users, the baseline group, are made in good faith. First-time editors are predicted to be 77.4\% good faith, a relatively minor difference of 5.7\% from IP and Tor editors. Our model predicts that registered editors are substantially higher in their good faith prediction of 97.7\%.

Our model of damaging edits in the second column of Table~\ref{tab:regression-dg} predicts that 41.3\% of Tor edits will be damaging. The model predicts that 39.9\% of IP editors will be damaging. And although this difference is statistically significant, it is not substantively so. Edits from first-time editors have a 33.8\% probability of being damaging (only 7.5\% lower). Contributions by registered editors are estimated to have only a 4.4\% chance of being damaging.
%This analysis provides support for the nature of the similarities between editors originating from Tor and other kinds of editors. 
% The model predicts that the probability of an edit made by an IP editor being damaging is nearly identical to the probability an edit made by a Tor editor being damaging ($\beta$=0.06).
Both models suggest that Tor edits are of similar quality to other editors without accounts and to registered contributors making their first edits.

\begin{table}[t] \centering 
  \caption{Logistic Regression Results: Prediction that an Edit was Good Faith, Damaging; Tor Editors are the Reference Category.} 
\label{tab:regression-dg}

\begin{tabular}{lcc}
 & Good Faith & Damaging \\
\hline
Intercept      & $0.90^{*}$       & $-0.35^{*}$       \\
               & $[0.85;\ 0.95]$  & $[-0.40;\ -0.30]$ \\
IP Editors     & $0.03$           & $-0.06^{*}$       \\
               & $[-0.03;\ 0.10]$ & $[-0.12;\ -0.00]$ \\
First Edits    & $0.33^{*}$       & $-0.32^{*}$       \\
               & $[0.26;\ 0.40]$  & $[-0.38;\ -0.26]$ \\
Reg Edits      & $2.87^{*}$       & $-2.73^{*}$       \\
               & $[2.73;\ 3.00]$  & $[-2.84;\ -2.63]$ \\
\hline
AIC            & 28709.73         & 37843.85          \\
BIC            & 28744.07         & 37878.20          \\
Log Likelihood & -14350.86        & -18917.93         \\
Deviance       & 9627.94          & 10486.61          \\
Num. obs.      & 39585            & 39594             \\
\hline
\multicolumn{3}{l}{\scriptsize{$^*$ 0 outside confidence interval. Ranges are 95\% confidence interval.}} \\
\end{tabular}

\end{table}
%%%%%RENOVATION PENDING ABOVE 




% \section{Tor users' behavior across other language editions}
%\section{Other Language Wikipedia editions}

%Wikipedia exists in hundreds of languages. These language editions are supported by different communities of administrators and users with varying guidelines and rules. In this section, we examine the behaviors of Tor users across five of the largest and most active Wikipedia language versions. We examined all Wikipedia language editions that ORES edit quality assessment models exist for in order to identify the top 5 languages in term of number of edits made through Tor.\footnote{\url{https://tools.wmflabs.org/ores-support-checklist/}} We found 6,020 Tor edits made on German Wikipedia (\emph{dewiki}) 1,632 edits made on French Wikipedia (\emph{frwiki}), 3,795 edits made on Russian Wikipedia (\emph{ruwiki}), and 1,129 made on Spanish Wikipedia (\emph{eswiki}), from 2007 to 2018. These correspond to 5 of the top 6 Wikipedia language editions in terms of number of edits in February 2019.\footnote{\url{https://en.wikipedia.org/wiki/List_of_Wikipedias}} With the exception of Spanish, these languages are the largest languages in countries that are mong the top 10 in terms of Tor relay usage.\footnote{\url{https://metrics.torproject.org/userstats-relay-table.html}}


%\begin{figure}[t]
%\includegraphics[width=8cm, %height=6cm]{figures/editsPerMonthStripes.png}
%\caption{Monthly edit trends by Tor users to different %language editions: English (enwiki), German (dewiki), %French(frwiki), Spain (eswiki), and Russian (ruwiki).}
%\label{fig:multilang-edittrend}
%\end{figure}
%Figure \ref{fig:multilang-edittrend} shows the LOESS smoothed number of edits made through Tor over time (similar to Figure \ref{fig:monthly-edits}). Because there were virtually no edits made after 2013, we omit the edits after 2013. Once again, we see spikes of edits indicative of ineffective ban mechanisms from 2008 to 2013. While the edits in German and Russian follow a similar trend to English, the contributions of Tor users in French and Spanish increase over time before the abrupt drop in 2013. The unlikely growth of Tor edits over time in these two languages could mean that interest in using Tor was increasing in these countries. 

%Figure \ref{fig:multilang-ores} shows the trends for the average likelihood of damaging and good faith edits across all five language editions. To visualize the difference in behaviors of Tor editors across multiple languages, we again show LOESS curves side-by-side. Compared to English, German, French, Russian, and Spanish Wikipedia receive higher probabilities of damaging edits.  
%Despite a gradual increase in the number of edits towards the end of 2012, the quality of edits in French language edition was getting significantly better. 
%This suggests that a positive development both in quantity and quality in the French-speaking , before their effort were completely stopped by the ban mechanism. On the other hand, the likelihood of damaging contribution on eswiki positively correlates with the amount of edits made. Spanish Wikipedia suffered from really high level of vandalism in the beginning, which sharply decreased in 2009, after the massive ban of Tor IP addresses started. As time went on, the damaging trend rose each time time there was an influx of edits slipped through the ban, and died down when the ban was reinforced.
%Figure \ref{fig:multilang-ores} also suggests that estimated levels of good faith edits in German Wikipedia are much higher than other languages. While Russian and Spanish decrease, English and French show an increase in good faith edits from Tor, especially toward the end of the period of study.

%To test the statistical evidence for these appearances, we construct a linear regression analogous to the one we developed for our English user comparison sets, assessing the relationship between time and both good faith and damaging predictions. Because ORES is trained separately on each language and is therefore subject to any expectations or conditions which differ by language, we fit each regression separately, although we combine the coefficients for display. Table \ref{tab:regression-LanguageDamaging} indicates that indeed English and French were becoming less damaging over time, and that this decrease was statistically significant, edits to German Wikipedia were becoming more damaging over time, while the changes in Spanish and Russian were not found to be statistically significant. Considering the good faith model, we see in Table \ref{tab:regression-LanguageGoodFaith} that French, English, and German edits were gauged to be increasingly good faith over time, while Russian and Spanish edits were gauged to be decreasingly made in good faith over time. This divergence in the direction of per-language trends suggests that the language populations using Tor may differ in their intentions and behavior.


%gives us a very interesting surprise, when displaying the prediction of good faith editing. Generally, the curves portraying the trends of frwiki, ruwiki, eswiki, and enwiki are in agreement with the prediction of damaging edits above: the more damaging the revisions are, the less likely that they were done in good faith. However, the prediction of contribution quality in dewiki tells a different story: even though these edits are likely to be damaging, with the confidence rating higher than 50\% throughout the timeline, ORES assesses that they are done almost completely in good faith. Unfortunately, we currently do not have the capacity to manually check the dataset for further insight.
%\begin{figure*}[t]
%\centering
%\includegraphics[width=15cm, height=12cm]{figures/byLanguageFacet.pdf}
%\caption{ORES prediction of Damaging and Good Faith edits, drawn as a non-parametric LOESS curve.}
%\label{fig:multilang-ores}
%\end{figure*}


==> oldcontentanalysis.tex <==
consulted the Wikipedia entry on assuming Good Faith to develop our approach to coding,\footnote{\url{https://en.wikipedia.org/wiki/Wikipedia:Assume_good_faith}} and examined whether the intent of an edit appeared to be consistent with community goals for building an encyclopedia. In determining if an edit was damaging or not, we also adopted community vocabulary and definitions: a damaging edit is one that, for any number of reasons internal to the norms of the community, should be reverted because it has made an article worse instead of better. We also gave ourselves the option to code an edit as ``in dispute'' in either category if we felt that a determination might be debatable within the Wikipedia community due the community's conflicting policies and priorities.

During the initial coding phase, we developed shared definitions of codes by using an iterative process to reach agreement. Each author coded 20 edits from a random dataset and then compared and discussed results. We then coded another 20 random sample of edits, and were able to achieve 100\% agreement after discussion. However, independent coding was more challenging due to the interpretive nature of the process. To assess our inter-rater reliability we used Krippendorff's alpha, which is appropriate for use when there are multiple coders and the data are nominal. This method yielded only marginal level of agreement for good/bad faith ($\alpha = 0.567$) and damaging or not damaging ($\alpha = 0.621$). 

\begin{table}[t]
\centering 
  \caption{Hand-labelling Assessment That an Article Edit Is Good Faith, Non-Damaging.} 
\label{tab:handcode}
\begin{tabular}{lccc}
 Sample Group & Good Faith & Non-Damaging & Size \\
\hline
\hline
 Tor & 66.5\% & 55.2\% & 330 \\
 IP & 65.3\% & 60.5\% & 249 \\
 First-time & 66.7\% & 55.6\% & 204 \\
 Registered & 90.8\% & 87.1\% & 172 \\
\hline
\multicolumn{3}{l}{\scriptsize} \\
\end{tabular}

\end{table}

\begin{table}[t]
\centering 
  \caption{Logistic Regression Results: Hand-coded Evaluation of Articles. First-time Editors are the Baseline.} 
  \label{tab:logitHand} 
\begin{tabular}{@{\extracolsep{5pt}}lcc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{2}{c}{\textit{Model:}} \\ 
\cline{2-3} 
\\[-1.8ex] & Good Faith & Non-Damaging \\ 
\hline \\[-1.8ex] 
 Registered & 2.862$^{***}$ & 2.327$^{***}$ \\ 
  & [1.83, 3.90] & [1.66, 3.00] \\ 
  & & \\ 
 IP & 0.024 & 0.301 \\ 
  & [-0.38, 0.43] & [-0.08, 0.68] \\ 
  & & \\ 
 Tor & $-$0.196 & $-$0.150 \\ 
  & [-0.57, 0.18] & [-0.50, 0.20] \\ 
  & & \\ 
 Constant & 0.875$^{***}$ & 0.357$^{**}$ \\ 
  & [0.57, 1.18] & [0.08, 0.64] \\ 
  & & \\ 
\hline \\[-1.8ex] 
Observations & 955 & 955 \\ 
Log Likelihood & $-$503.064 & $-$565.921 \\ 
Akaike Inf. Crit. & 1,014.128 & 1,139.842 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{2}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01}.\\ & \multicolumn{2}{r} {95\% confidence intervals shown. }
\end{tabular} 
\end{table} 

The results of our hand-coding are summarized in Table \ref{tab:handcode}. We observe that Tor editors contribute at a Non-Damaging rate that is somewhat better than our comparison sets of IP editors and First-time editors, with 66.1\%, 60.8\% and 58.9\% Non-Damaging respectively, while experienced editors have a Non-Damaging rate of 94.8\%. 
To provide a statistical test of the differences between the groups shown in Table \ref{tab:handcode}, we fit logistic regression models on our measures of quality with the editor group as our independent variable. Table \ref{tab:logitHand} reports the coefficients from this analysis with 95\% confidence intervals in brackets. The result suggests that while experienced editors were more likely to be Good Faith, Non-Damaging contributors, we were not able to detect statistically significant differences between First-time editors, IP, and Tor editors. This analysis supports a conclusion that individuals from these three groups act in a Good Faith, Non-Damaging manner at about the same rate.
